Predicting What You Already Know Helps: Provable Self-Supervised Learning

Self-supervised representation learning solves auxiliary prediction tasks (known as pretext tasks) without requiring labeled data to learn useful semantic representations. These pretext tasks are created solely using the input features, such as predicting a missing image patch, recovering the color channels of an image from context, or predicting missing words in text; yet predicting this \textit{known} information helps in learning representations effective for downstream prediction tasks. We posit a mechanism exploiting the statistical connections between certain {\em reconstruction-based} pretext tasks that guarantee to learn a good representation. Formally, we quantify how the approximate independence between the components of the pretext task (conditional on the label and latent variables) allows us to learn representations that can solve the downstream task by just training a linear layer on top of the learned representation. We prove the linear layer yields small approximation error even for complex ground truth function class and will drastically reduce labeled sample complexity. Next, we show a simple modification of our method leads to nonlinear CCA, analogous to the popular SimSiam algorithm, and show similar guarantees for nonlinear CCA.

==> CI.tex <==
% !TEX root = gaussian_model.tex

\section{Guaranteed recovery with conditional independence}

%\revise{Section and subsection titles should only have first letter capitalized according to instructions.}
%We are interested in variable $(x_1,x_2,\by)\in\Rr^{d_1+d_2+k}$, where $x_1\in\R^{d_1}, x_2\in\Rr^{d_2}$ and $y\in\Rr^k$. For simplicity, we assume $X_1,X_2$ and $Y$ to be zero mean random variables.  % and assume that $(x_1,x_2,\by)$ is jointly gaussian with mean 0.
%Let $\bSigma\in\Rr^{(d_1+d_2+k) \times (d_1+d_2+k)}$ denote the covariance of the joint distribution $(X_1,X_2,Y)$. Let $\bSigma_{X_1X_2}$ be the covariance matrix between $X_1$ and $X_2$ and vice versa for all pairs of random variables among them.

%We first consider the setting where we only use linear functions for predictions. Note when $X_1,X_2,Y$ are jointly Gaussian, their conditional expectation is simply linear function.

In this section, we focus on the case when input $X_1$ and pretext target $X_2$ are conditional independence given the downstream label $Y$.
\revise{Discussion about general recipe, i.e. find an expression for the optimal $\psi^*$ for pretext task, use conditional independence to upper bound $e_{\apx}(\psi^*)$, analyze sample complexity on downstream task. As a warm up, we instantiate this in the case of gaussian data to highlight the important steps in the analysis and to quantify the benefits of this self-supervised learning. We then show how conditional independence is useful in the more general case.}

\paragraph{Data assumption. } Let $Y=f^*(X_1)+N$, where $f^*=\E[Y|X_1]$, and therefore residual $N$ is mean 0. We assume $N$ is a subgaussian random vector with $\psi_2$-norm %\jz{what is $\psi_2$ here?} 
of $\sigma$. For downstream task we have access to $n_2$ i.i.d. samples $(\bx_1^{(1)}, \by^{(1)}), \cdots,(\bx_1^{(n_2)}, \by^{(n_2)}) $ drawn from joint distribution with density $P_{X_1Y}$. For convenience, we express these $n$ samples collectively as an input matrix $\bX_1^{\down} \in \R^{n\times d_1}$ and an output matrix $\bY\in \R^{n_2\times k}$. We overload the representation function $\psi(\bX_1^{\down})=[\psi(\bx_1^{(1)})|\psi(\bx_1^{(2)})\cdots |\psi(\bx_1^{(n)})]^\top \in \R^{n_1\times d_2}$ that is applied row-wisely on each sample.    
For simplicity, we assume non-degeneracy in each random variable: $\bSigma_{X_iX_i}$ and $\bSigma_{YY}$ are full rank. 


\subsection{Warm-up: jointly Gaussian variables}
As a warm-up, we first look at the case when $X_1,X_2,Y$ are jointly Gaussian, and therefore the optimal regression functions are all linear, i.e., $\E[Y|X]=\E^L[Y|X]$. For simplicity we assume data is centered: $\E[X_i]=0$ and $\E[Y]=0$. In this case, all relationship among random variables could be captured by the (partial) covariance matrix. Therefore it is easy to quantify the conditional independence property and establish the necessary and sufficient conditions that makes $X_2$ a reasonable pretext task.  

\begin{assumption} (Jointly Gaussian)
\label{assumption:jointly_gaussian}
	$X_1,X_2,Y$ are jointly Gaussian.
\end{assumption}

\begin{assumption} (Conditional independence)
	\label{assumption:conditional_independence}
	$X_1\bot X_2|Y$.
\end{assumption}



\begin{claim}
Under Assumption \ref{assumption:jointly_gaussian}, the representation function and optimal prediction that minimize the population risk can be expressed as follows:
	\begin{align}
\psi^*(\bx_1):=\E^L[X_2|X_1=\bx_1] &= \bSigma_{X_2X_1}\bSigma_{X_1X_1}^{-1}\bx_1  \\
\text{Our target }f^*(\bx_1):=\E^L[Y|X_1=\bx_1] & = \bSigma_{YX_1}\bSigma_{X_1X_1}^{-1}\bx_1.
\end{align}
%\revise{call this $\psi^*$ for consistency?}
\end{claim}

Our prediction for downstream task with representation $\psi^*$ will be:
$g(\cdot) :=  \E^L[Y|\psi^*(X_1)] $. 
Recall the partial covariance matrix between $X_1$ and $X_2$ given $Y$ is:
$$ \bSigma_{X_1X_2| Y} \equiv \bSigma_{X_1X_2}-\bSigma_{X_1Y}\bSigma_{YY}^{-1}\bSigma_{YX_2}.   $$

This partial covariance matrix captures the correlation between $X_1$ and $X_2$ given $Y$. For random variables that are jointly Gaussian, CI is equivalent to $ \bSigma_{X_1X_2| Y} =0 $. %Meanwhile when $\bSigma_{X_1X_2| Y}$ is of small norm, it means given $Y$, $X_1$, and $X_2$ has little correlation. When $\bSigma_{X_1X_2| Y} $ is low rank, it means there exists some additional latent variable $Z$ such that $ \cov(X_1, X_2|\bar Y)=0,$ where $\bar Y = [Y,Z]$. 

In the following we will analyze the approximation error based on the property of this partial covariance matrix.




\begin{lemma}
	\label{lemma:linear_CI} 
	Under Assumption \ref{assumption:jointly_gaussian}, \ref{assumption:conditional_independence}, if $\bSigma_{X_2Y}$ is of rank $k$, then we have $e_{\apx}(\psi^*)=0$.
\end{lemma}

\begin{remark}
	$\bSigma_{X_2Y} $ being full column rank infers that $\E[X_2|Y]$ is of rank $k$, i.e., $X_2$ depends on all directions of $Y$. This roughly means that $X_2$ captures all directions of information of $Y$. This is a necessary assumption for $X_2$ to be a reasonable pretext task for predicting $Y$. %, since otherwise one will inevitably lose information of $Y$ from the pretext task.  
\end{remark}

It is easy to generalize the result when $Y$ only reduces the rank of partial covariance matrix instead of making it exactly $0$. 

\begin{assumption}[Conditional Independent Given Latent Variables]
	\label{assumption:CI_with_latent_variables}
	Assume there exists some latent variable $Z\in \R^m$ such that $X_1\bot X_2|\bar Y $, and $\bSigma_{X_2\bar Y}$ is of rank $k+m$, where $\bar Y = [Y,Z]$. 
	%$\sigma_k(P_{\bSigma_{X_1Y}}\bSigma_{X_1X_2})\geq C, $ for some positive $C$. Here the operator $P_A = A(A^\top A)^\dagger A^\top$ is the projection onto the column space of matrix $A$.  
\end{assumption}

Assumption \ref{assumption:CI_with_latent_variables} makes sure we introduce some reasonable latent variables that capture the joint information between $X_1$ and $X_2$ apart from $Y$. $\cov(X_2, \bar Y)$ to be full rank is to say all directions of $\bar Y$ is useful in predicting $X_2$, and therefore $Z$ is not redundant. (For instance, when $Z=X_1$ the assumption is true, but $Z$ is not the minimal latent information we want to add.) 
%This is a natural and necessary condition for $X_2$ to be a reasonable pretext task and the introduction of latent variable $Z$ is not redundant. 
Notice it implicitly requires $d_2\geq k+m$. 

\begin{corollary}
	\label{coro:linear_CI_with_latent_variable} 
	Under Assumption \ref{assumption:jointly_gaussian}, \ref{assumption:CI_with_latent_variables},  the approximation error $e_{\apx}(\psi^*)$ is 0. 
\end{corollary}

Next we consider the estimation error. In other words, how many samples do we require to learn a good prediction function $g(\bx_1)=W\psi^*(\bx_1)$ that generalizes. 
With finite samples $\bX_1,\bY$ with each sample $(\bx_1^{(i)},\by^{(i)}) \sim P_{X_1Y}$, we do linear regression on top of the learned representation $\psi^*$:
\begin{equation*}
\hat \bW\leftarrow \argmin_{W} \frac{1}{2n}\|\bY-\psi^*(\bX_1)W\|_F^2, 
\end{equation*}
We are interested in the excess risk that measures generalization: %\revise{Again $\ER_\psi(\hat \bW)$ or $\ER(\hat \bW; \psi)$?}
\begin{equation*}
\ER_{\psi^*}(\hat \bW) := \E \|f^*(X_1) - \hat\bW^\top \psi^*(X_1) \|_2^2.
\end{equation*}

\begin{theorem}
	\label{thm:linear_CI} 
	Fix a failure probability $\delta\in (0,1)$. Under Assumption \ref{assumption:jointly_gaussian},\ref{assumption:conditional_independence}, if additionally $n\gg k+\log(1/\delta)$, the excess risk of the learned predictor $\bx_1\rightarrow \hat \bW\psi^*(\bx_1)$ on the target task satisfies
	\begin{equation*}
	\ER_{\psi^*}(\hat \bW) \lesssim \frac{\Trace(\bSigma_{YY|X_1})(k  + \log (k/\delta))}{n},  
	\end{equation*} 
	with probability at least $1-\delta$. %Here $\sigma^2=\Trace(\bSigma_{YY|X_1})$.
\end{theorem}
Here $\bSigma_{YY|X_1}\equiv \bSigma_{YY}-\bSigma_{YX_1}\bSigma_{X_1X_1}^{-1}\bSigma_{X_1Y}$ captures the noise level. It is the covariance matrix of the residual term $Y-f^*(X_1)=Y-\bSigma_{YX_1}\bSigma_{X_1X_1}^{-1}X_1$. Compared to directly using $X_1$ to predict $Y$, self-supervised learning reduces the sample complexity from $\cO(d_1)$ to $\cO(k)$. If a weaker assumption \ref{assumption:CI_with_latent_variables} is satisfied, simply replace $k$ by $k+m$ will suffice. 
%\revise{Discussion about what this result means}

\subsection{General random variables}
Next we move on to general setting where $\E[Y|X_1]$ and $\E[X_2|X_1]$ can be arbitrary functions of $X_1$. 
\begin{assumption}
	\label{assump:independence}
	Let $X_1\in \R^{d_1},X_2\in \R^{d_2}$ be random variables from some unknown distribution. Let label $Y\in \cY\subset \R^k$ be a discrete random variable with $c=|\cY|<d_2$. We assume conditional independence: $X_1\bot X_2|Y$. 
	\revise{Use different notation than $c$? $c$ looks more like a constant and might be confusing. Can use $k$ instead since $\R^k$ does not seemed to be used anywhere.}
\end{assumption}
Here $Y$ can be interpreted as the multi-class labels where $c$ is the number of classes. For regression problems, one can think about $Y$ as the discretized values of continuous labels. 
\revise{Mention that $\psi^*(X_1) = \E[X_2|X_1]$ is the optimal solution, since it was not discussed yet I think.}
\begin{lemma}
	\label{lemma:discrete_case_CI}
	Suppose random variables $X_1,X_2,Y$ satisfy Assumption \ref{assump:independence}, and additionally matrix $\bA \in \R^{\cY\times d_2} $ with $\bA_{y,:} := \E[X_2|Y=\by]$ is of rank $c=|\cY|$. %\jz{mention what is $\bA$ here?}
	Then $e_\apx(\psi^*) = 0$. 
\end{lemma}


\begin{remark}
	This lemma suggests that with self-supervised representation learning procedure $\psi^*(X_1)=\E[X_2|X_1]$, the downstream task prediction of $Y$ is a linear function of $\psi^*$. And the linear map is at most of rank $|\cY|$.
	\revise{Is the rank covered in this lemma?}
	%For feature map with universal property, we will have	$\E[Y|X_1] = \E^L [Y|\phi_1(X_1)] = (w^*)^\top \psi(X_1)$. Then our conclusion will be we could learn $\E[Y|X_1]$ by using linear regression to learn $Y$ from $\psi(X_1)$. 
\end{remark}
To estimate the sample complexity under general function class, we need to assume the representation has some good concentration property. First we introduce the whitening of $\psi^*(X_1)$ to reduce scaling factors. Assume $\E[\psi^*(X_1)]=0$ and write $\bSigma_{\psi} = \E[\psi^*(X_1)\psi^*(X_1)^\top]$. Let random variable $U=\bSigma_{\psi}^{-1/2}\phi(X_1)$. Then it satisfies $\E[U]=0$ and $\var{U}=\bI$.  

\begin{assumption}
	\label{assumption:subgaussian_psi}
Write $\bSigma_{\psi} = \E[\psi^*(X_1)\psi^*(X_1)^\top]$. We assume the whitened feature variable $U:=\bSigma_{\psi}^{-1/2}\psi^*(X_1)$ is a $\rho^2$-subgaussian random variable. %\footnote{A random vector $\bx$ is called $\rho^2$-subgaussian if for any fixed unit vector $\bv$ of the same dimension, the random variable $\bv^\top \bx$ is $\rho^2$-subgaussian, i.e., $\E[e^{s\cdot\bv^\top(\bx-\E[\bx])}]\le e^{s^2\rho^2/2}$ ($\forall s\in\R$). \jz{Seems removable}}  
Residual term $N=Y-\E[Y|X_1]$ satisfies $\E[\|N\|^2|X_1]\leq \sigma^2.$ % $k\sigma^2$-subgaussian.
\end{assumption}
We note that all bounded random variables satisfy sub-gaussian property. %For multi-classification problems $N$ is naturally bounded 

\begin{theorem}(General Conditional Independence)
	\label{thm:CI_nonlinear_sample_complexity}
	Fix a failure probability $\delta\in (0,1)$, under the same assumption as Lemma \ref{lemma:discrete_case_CI} and Assumption \ref{assumption:subgaussian_psi}, if additionally $n\gg \rho^4(c+\log(1/\delta))$, then the excess risk of the learned predictor $\bx_1\rightarrow \hat\bW^\top \psi(\bx_1)$ on the downstream task satsifies:
	\begin{equation*}
	\ER[\hat \bW] \lesssim \frac{c+\log(c/\delta)}{n}\sigma^2. 
	\end{equation*}
\end{theorem}
%\qi{for binary $Y$, does this $f^*(X_1)+\epsilon$ assumption make sense?... shall we change this result from regression to classification tasks? }


\begin{remark}
	This analysis assumes we could perfectly learn $\psi=\E[X_2|X_1]$ without considering the number of samples on the self-supervised learning part, since we could have arbitrary number of unlabeled data. Here by sample complexity we refer to the input data with labels $X_1,Y$. We will analyze the robustness in learning the representation learning later.
\end{remark}

%\begin{remark}
%	To understand the benefits of using $\psi(X_1)$ instead of $X_1$ to predict $Y$, we note the following two points. On one hand, it is much easier to learn a linear model instead of an unknown model in $\cF_1$, and we have $\E^L[Y|\psi(X_1)]=\E[Y|X_1]$. On the other hand, it is easy to show $\var{Y|X_1}\geq \var{Y|\psi(X_1)}$.
%\end{remark}


\revise{Add a subsection for $\psi$ being linear function of finite dimensional features? It is easy to present and understand. Section 4 will bring everything together.}
\subsection{Linear function}
Here we consider the simple case where $\psi(\bx_1) = \bA\phi_1(\bx_1)$ is assumed to be a linear function of some given features $\phi_1$ of $\bx_1$, where $\phi_1:\cX_1\rightarrow\R^{d_1}$.
Thus we will have $\psi^*(\bx_1) = \bA^*\phi_1(\bx_1)$, where
\begin{align*}
	\bA^* = \arg\min_{\bA\in\R^{d_1\times d_2}} \E_{X_1,X_2} [\|X_2 - \bA\phi_1(X_1)\|^2]
\end{align*}
Even in this case we can show the benefit of conditional independence, by showing that $\psi^*$ will perform better than the original features $\phi_1$ on downstream task.
Note that since $\psi^*$ is a linear function of $\phi_1$, it cannot have smaller approximation error than $\phi_1$.
However we show that conditional independence will ensure that $\psi^*$ has the same approximation error as $\phi_1$, but enjoys much better sample complexity.
\begin{claim}
	$\psi^*(\bx_1) = \bSigma_{X_2\phi_1}\bSigma_{\phi_1\phi_1}^{-1}\bx_1$
\end{claim}

\begin{lemma}
	\label{lemma:linear_case_CI}
	Suppose random variables $X_1,X_2,Y$ satisfy Assumption \ref{assump:independence}, and additionally matrix $\bA \in \R^{\cY\times d_2} $ with $\bA_{y,:} := \E[X_2|Y=\by]$ is of rank $c=|\cY|$.
	Then $e_\apx(\psi^*) = e_{\apx}(\phi_1)$. 
\end{lemma}

\begin{theorem}(Linear Conditional Independence)
	\label{thm:CI_linear_sample_complexity}
	\revise{Need to fix this statement, define subgaussian assumption in this case, and additional Sham assumption.}
%	Fix a failure probability $\delta\in (0,1)$, under the same assumption as Lemma \ref{lemma:linear_case_CI} and Assumption \ref{assumption:subgaussian_psi}, if additionally $n\gg \rho^4(c+\log(1/\delta))$, then the excess risk of the learned predictor $\bx_1\rightarrow \hat\bW^\top \psi(\bx_1)$ on the downstream task satsifies:
	\begin{equation*}
		\ER[\hat \bW] \lesssim e_{\apx}(\phi_1) + \frac{c+\log(c/\delta)}{n}\sigma^2. 
	\end{equation*}
\end{theorem}

\revise{Comment that everywhere $\bx_2$ can be replaced with $\phi_2(\bx_2)$, only full rank-ness needs to be satisfied.}

==> abs2.tex <==
\begin{abstract}
Self-supervised learning learns useful representations via supervised learning on a set of pretext tasks. 
\end{abstract}

==> experiments_nlp.tex <==
% !TEX root = colt2021-SSL.tex


%\begin{wrapfigure}{r}{0.5\textwidth}
%\label{fig:exp-sst}
%\vspace{-20pt}
%\includegraphics[width=0.5\textwidth]{figures/bow_rand300_sst_clf_.png}
%\vspace{-10pt}
%\caption{Classification accuracy on SST of baseline $\phi_1(\bx_1)$, i.e. bag-of-words, and learned $\psi(\bx_1)$ for the two settings.}\label{fig:exp-sst}
%\vspace{-10pt}
%\end{wrapfigure}





%\revise{Do we need the IMDB case? It is not much better than $\phi_1$. Do ER instead of absolute error?}
%
%\begin{figure}
%    \centering     %%% not \center
%    \hspace{-3pt}
%    \subfigure{\includegraphics[width=0.49\textwidth]{figures/bow_rand300_sst_reg_.png}}
%    \hspace{-10pt}
%    \subfigure{\includegraphics[width=0.49\textwidth]{figures/bow_rand300_sst_clf_.png}}
%    \hspace{-10pt}
%    \caption{Performance on SST of baseline $\phi_1(\bx_1)$, i.e. bag-of-words, and learned $\psi(\bx_1)$ for the two settings. (a) regression MSE (b) classification accuracy (between 0 and 1).}\label{fig:exp-sst}
%    \vspace{-15pt}
%\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Appendix reference, lower-case.
\def\apxref#1{appendix~\ref{#1}}
% Appendix reference, capital.
\def\Apxref#1{Appendix~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

%%%%%% Custom %%%%%%
% Reference to a theorem, lower and upper case.
\def\thmref#1{theorem~\ref{#1}}
\def\Thmref#1{Theorem~\ref{#1}}
% Reference to a lemma, lower and upper case.
\def\lemref#1{lemma~\ref{#1}}
\def\Lemref#1{Lemma~\ref{#1}}
% Reference to a definition, lower and upper case.
\def\defref#1{definition~\ref{#1}}
\def\Defref#1{Definition~\ref{#1}}
% Reference to two equations, upper case
\def\twoEqref#1#2{Equations \ref{#1} and \ref{#2}}
%%%%%%%%%%%%%%%%%

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
%\newcommand{\train}{\mathcal{D}}
%\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
%\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> robust.tex <==
% !TEX root = gaussian_model.tex
\section{Robust analysis}
\paragraph{Just a proof sketch:} Suppose $\tilde{\psi}:\R^{d_1}\rightarrow\R^{d_2}$ is the learned function that will be used to predict a downstream task $f^*(x) = A^*\psi(x) + \eta$, where $\psi(x_1)=\E[X_2|x_1]$, $A^*\in\R^{k\times d}$ and $\eta$ is a zero mean and subgaussian random variable.
Denote the risk of function $g$ as $\ell(g)=\min_{A\in\R^{k\times d}}\E[\|f^*(x_1)-Ag(x_1)\|^2]$.

\begin{lemma}
Suppose $\tilde{\psi}:\R^{d_1}\rightarrow\R^{d_2}$ is such that $\E\|\tilde{\psi}(X_1)-\psi(X_1)\|^2\le\epsilon$, where and suppose $\|\psi(x)\|\le R,\forall x\in\R^{d_1}$, then for a target function $f^*$ as defined above, we have
\begin{align*}
	\ell(\tilde{\psi})-\ell(\psi)\le\lambda_{max}(A^*)\epsilon
\end{align*}
For $\Psi=\E[\psi(X_1)\psi(X_1)^\top]\in\R^{d_2\times d_2}$, $\tilde{\Psi}=\E[\tilde{\psi}(X_1)\tilde{\psi}(X_1)^\top]$, let $\Psi=V\Lambda V^\top$ and $\tilde{\Psi}=\tilde{V}\tilde{\Lambda}\tilde{V}^\top$ be the eigen decompositions, where $\Lambda = diag(\lambda_1,\dots,\lambda_{d_2})$ and $\tilde{\Lambda}=diag(\tilde{\lambda}_1,\dots,\tilde{\lambda}_{d_2})$. Then we have
\begin{align*}
	|\lambda_i - \tilde{\lambda}_i| &= \cO(\epsilon + R\sqrt{\epsilon}),~~\forall i\in[d_2]\\
	\|V_k-\tilde{V}_kO_k\|_F &= O\left(\frac{\epsilon + R\sqrt{\epsilon}}{\lambda_k-\lambda_{k+1}}\right)
\end{align*}
where $V_k,\tilde{V}_k\in\R^{d_2\times k}$ are first $k$ eigenvectors and $O_k\in\R^{k\times k}$ is an orthogonal matrix.
\end{lemma}
\begin{proof}
To prove the first part, we notice that $\ell(\tilde{\psi})-\ell(\psi)=\min_A\E[\|A^*\psi(X_1)-A\tilde{\psi}(X_1)\|^2 \le \E[\|A^*\psi(X_1)-A^*\tilde{\psi}(X_1)\|^2\le\E[\lambda_{max}(A^*)\|\psi(X_1)-\tilde{\psi}(X_1)\|^2]\le\lambda_{max}(A^*)\epsilon$

For the second part, for $\Delta(X_1)=\tilde{\psi(X_1)}-\psi(X_1)$, we have $\E[\|\Delta(X_1)\|^2]\le\epsilon$ from the unsupervised loss condition. Then we get
\begin{align*}
	\tilde{\Psi}
	&=\E[\tilde{\psi}(X_1)\tilde{\psi}(X_1)^\top]\\
	&=\E[\psi(X_1)\psi(X_1)^\top] + \E[\Delta(X_1)\Delta(X_1)^\top] + \E[\Delta(X_1)\psi(X_1)^\top] + \E[\psi(X_1)\Delta(X_1)^\top]\\
	&=\Psi + \E[\Delta(X_1)\Delta(X_1)^\top] + \E[\Delta(X_1)\psi(X_1)^\top] + \E[\psi(X_1)\Delta(X_1)^\top]\\
	&\coloneqq \Psi + E
\end{align*}
where $E$ is the difference matrix.
The forbenius norm of $E$ can be bounded by 
\begin{align*}
	\|E\|_F
	&= \|\E[\Delta(X_1)\Delta(X_1)^\top] + \E[\Delta(X_1)\psi(X_1)^\top] + \E[\psi(X_1)\Delta(X_1)^\top]\|_F\\
	&\le \E[\|\Delta(X_1)\Delta(X_1)^\top\|_F] + \E[\|\Delta(X_1)\psi(X_1)^\top\|_F] + \E[\|\psi(X_1)\Delta(X_1)^\top|_F]\\
	&\le \E[\|\Delta(X_1)\|^2] + 2\E[\|\Delta(X_1)\|\|\psi(X_1)\|]\\
	&\le \epsilon + 2R\E[\|\Delta(X_1)\|]\\
	&\le \epsilon + 2R\sqrt{\E[\|\Delta(X_1)\|^2]} \le \epsilon + 2R\sqrt{\epsilon}
\end{align*}
Weyl's inequality along with the fact that $\tilde{\Psi}=\Psi+E$ to get $\lambda_i(\tilde{\Psi})\in[\lambda_i(\Psi)-\|E\|_F,\lambda_i(\Psi)+\|E\|_F]$ for every $i$.

For the third part, we use a variant of Davis-Kahan theorem to argue that the eigenspaces also align.
Let $\Psi=VSV^T$ and $\tilde{\Psi}=\tilde{V}\tilde{S}\tilde{V}^T$ be the eigen decompositions of $\Psi$ and $\tilde{\Psi}$ respectively.
%Let $V_k$, $S_k$ correspond to the top $k$ eigenvalues and eigenvectors; similarly define $\tilde{V}_k$ and $\tilde{S}_k$.
Using Theorem 2 from \cite{yu2015useful}, we get that there exists an orthogonal matrix $O\in\R^{k\times k}$ such that $\|\tilde{V}_k-V_kO\|_F\le \frac{2\sqrt{2}\|E\|_F}{\lambda_k-\lambda_{k+1}}$.
{\color{red} This basically shows that projection matrix of top $k$ eigenvalues of $\tilde{\Psi}$ almost aligns with the projection matrix of $\Psi$, while the remaining $d_2-k$ directions have $O(\|E\|_F)$ eigenvalues.}
This completes the proof.
\end{proof}
Using the above lemma, we see that since $\Psi$ is low rank, $\tilde{\Psi}$ is almost low rank and solving ridge regression with appropriate regularization will give similar sample complexity.
{\color{red} need to complete}.

\jnote{1)Minor thing: Seems that you might try to show directly $P_{\linspan(\Psi)} \approx P_{\linspan(\tilde \Psi)}$, so at least condition numbers might be avoided (not clear to me it can be avoided but would be nice) \\ 
2) If $A_{21}=0$, then may as well consider $d_2=2^k$ where $k$ is number of bits in $y$ (so $2^k$=num classes). In this case, I don't think you ever need to consider ridge, instead would do regular least squares. \\
3) If $A_{21} \neq 0$, then $\Psi, \tilde \Psi $ are full rank of $d_2$.  There are 3 sources of error: approximation , bias and variance.
It's not clear to me we even need ridge regression in this case since this can only help the bias-variance tradeoff not approximation. You can probably just achieve the same tradeoff as ridge just by choosing $d_2$ small. E.g. say $y$ is binary, then I think the optimal choice of $d_2=1$. The case where ridge helps is if you chose $d_2\gg 1$, and then ridge could get you a better bias-variance tradeoff. But I don't think it can be better than just choosing $d_2$ correctly?
\\
EDIT: Seems you should always just do SVD on $\tilde \Psi$ to reduce it to rank 1 (or whatever the $2^{bits(y)}$).
}
